A reddening-free method to estimate the $^{56}$Ni mass of Type Ia supernovae

The increase in the number of Type Ia supernovae (SNe\,Ia) has demonstrated that the population shows larger diversity than has been assumed in the past. The reasons (e.g. parent population, explosion mechanism) for this diversity remain largely unknown. We have investigated a sample of SNe\,Ia near-infrared light curves and have correlated the phase of the second maximum with the bolometric peak luminosity. The peak bolometric luminosity is related to the time of the second maximum (relative to the {\it B} light curve maximum) as follows : $L_{max}(10^{43} erg s^{-1}) = (0.039 \pm 0.004) \times t_2(J)(days) + (0.013 \pm 0.106)$. $^{56}$Ni masses can be derived from the peak luminosity based on Arnett's rule, which states that the luminosity at maximum is equal to instantaneous energy generated by the nickel decay. We check this assumption against recent radiative-transfer calculations of Chandrasekhar-mass delayed detonation models and find this assumption is valid to within 10\% in recent radiative-transfer calculations of Chandrasekhar-mass delayed detonation models. The $L_{max}$ vs. $t_2$ relation is applied to a sample of 40 additional SNe\,Ia with significant reddening ($E(B-V) >$ 0.1 mag) and a reddening-free bolometric luminosity function of SNe~Ia is established. The method is tested with the $^{56}$Ni mass measurement from the direct observation of $\gamma-$rays in the heavily absorbed SN 2014J and found to be fully consistent. Super-Chandrasekhar-mass explosions, in particular SN\,2007if, do not follow the relations between peak luminosity and second IR maximum. This may point to an additional energy source contributing at maximum light. The luminosity function of SNe\,Ia is constructed and is shown to be asymmetric with a tail of low-luminosity objects and a rather sharp high-luminosity cutoff, although it might be influenced by selection effects.

==> ana.tex <==
%\section{Analysis}
The integrated flux emitted by an SN~Ia in the UV, optical and NIR traces the comptonization of the $\gamma-$rays emitted through the $^{56}$Ni $\rightarrow$  $^{56}$Co $\rightarrow$ $^{56}$Fe decay chain \citep[see][]{Nadyozhin1994}.
As the SN emits most of its flux in the UV to NIR passbands, the "UVOIR bolometric flux" represents a physically meaningful quantity \citep{Suntzeff1996}

We selected a low-reddening sample of objects with a host extinction less than $\rm 0.1 mag$ . This makes our measurements less sensitive to the reddening law. 
We constructed UBVRIJH bolometric light curves for objects with sufficient photometry near maximum light in the optical and the NIR. The $K$ band data was not included since only few SN~Ia have well-sampled $K$ band light curves. For a few SN~Ia with sufficient $K$ light curves we calculated the fraction of the flux emitted in $K$ and determined it to be around $1-3 \%$. Therefore, the exclusion of the $K$-flux results in only a minor uncertainty.  


The small reddening correction following CCM was applied to our data before integrating over the available passbands and the uncertainty propagated into the bolometric flux. We use a distance scale of $H_0=70$~$km$~$s^{-1}$~$Mpc^{-1}$ and the assumed distances are indicated in Table~\ref{tab:mni}. For the nearby SN~Ia with distance measurements provided through direct methods (e.g. Cepheid stars, Tully-Fisher relation) we made sure to employ the same distance scale. 

%The magnitudes were corrected 
%for reddening using a CCM reddening law for each filter. The values for the extinction are presented in Table \ref{tab:mni}. The uncertainty in the reddening estimate was propagated into the calculation of the bolometric flux. Using zero-points in the given filters, the magnitudes were converted to fluxes. The data in the different filters is interpolated, instead of using a reference filter. The filters are integrated using the trapezoidal rule.
%The resulting light curve, in ergs/$cm^2$/s  was converted into an absolute bolometric light curve  by using the distances of the SN derived from the host galaxy redshift. 

%Since all distances are scaled to an $H_0=70 km s^{-1} Mpc ^{-1}$ the errors in the luminosity distance are only affected by the relative errors in the distance moduli (see Table \ref{tab:mni} for values and uncertainty estimates). For objects not in the Hubble flow, we use distance measurements from published estimates (which use others methods e.g. Cepheid, Tully-Fisher relation etc.). 

We restricted the analysis to SN~Ia with filter coverage from $u$ to $H$ filters and good temporal coverage around the bolometric maximum.

\input{tab/sn_samp_lr.tex}

==> tab/yj_ni.tex <==
\begin{table}
\begin{minipage}{70mm}
\begin{center}
\footnotetext{$^a$:$\cdot 10^{43} erg s^{-1}$}
\caption{$M_{Ni}$ measurements for the complete sample of objects with $t_2$ measurements in both $Y$ and $J$ bands.}
\begin{tabular}{llcrr}
\hline
SN & $L_{max}^{a}$ (J)	& $\sigma$ & $L_{max}^{a}$ (Y) & $\sigma$ \\
\hline
1980N & 0.91 & 0.13 &\ldots & \ldots \\
1981B & 1.32 & 0.15 &\ldots & \ldots\\
1998bu & 1.23 & 0.14 &\ldots & \ldots\\
1999ac & 1.12 & 0.14 &\ldots & \ldots\\
1999ee & 1.42 & 0.16 &\ldots & \ldots \\
2000E & 1.31 & 0.16 &\ldots & \ldots\\
2000bh & 1.37 & 0.15 &\ldots & \ldots\\
2001bt & 1.17 & 0.13 &\ldots & \ldots\\
2001cn & 1.24 & 0.14 &\ldots & \ldots\\
2001cz & 1.40 & 0.16 &\ldots & \ldots\\
2001el & 1.29 & 0.15 &\ldots & \ldots\\
2002bo & 1.12 & 0.13 &\ldots & \ldots\\
2003cg & 1.24 & 0.14 &\ldots & \ldots\\
2003hv & 0.92 & 0.12 &\ldots & \ldots \\
2004ey	&	1.21	&	0.19	&	1.31	&	0.20	\\
2004gs	&	0.93	&	0.16	&	0.91	&	0.16	\\
2004gu	&	1.46	&	0.22	&	1.54	&	0.22	\\
2005al	&	1.05	&	0.18	&	1.04	&	0.18	\\
2005na	&	1.35	&	0.20	&	1.13	&	0.19	\\
2006D	&	1.05	&	0.18	&	1.01	&	0.18	\\
2006ax	&	1.32	&	0.20	&	1.36	&	0.21	\\

2006et	&	1.33	&	0.22	&	1.35	&	0.20	\\
2006gt 	& 0.85 		& 0.11 &\ldots & \ldots\\
2006hb	&	0.79	&	0.17	&	0.72	&	0.15	\\
2006kf	&	1.01	&	0.17	&	1.07	&	0.10	\\
2007S	&	1.46	&	0.21	&	1.52	&	0.23	\\
2007af	&	1.22	&	0.19	&	1.23	&	0.19	\\
2007as	&	1.02	&	0.22	&	0.94	&	0.17	\\
2007bc  &\ldots & \ldots & 1.16 &  0.2 \\
2007bm	&	1.15	&	0.17	&	1.32	&	0.20	\\
2007ca  &\ldots & \ldots & 1.38 &  0.22 \\
2007if  &\ldots & \ldots & 1.34 & 0.22 \\
2007jg  &\ldots & \ldots & 1.12 & 0.2  \\
2007le	&	1.27	&	0.20	&	1.31	&	0.20	\\
2007nq	&	0.98	&	0.18	&	0.94	&	0.17	\\
2008C	&	1.33	&	0.21	&	1.23	&	0.19	\\
\hline
\end{tabular}
\end{center}
\end{minipage}
\label{tab:yj}
\end{table}
